Stochastic Galerkin finite volume shallow flow model: well-balanced treatment over uncertain topography

Stochastic Galerkin methods can quantify uncertainty at a fraction of the computational expense of conventional Monte Carlo techniques, but such methods have rarely been studied for modelling shallow water flows. Existing stochastic shallow flow models are not well-balanced and their assessment has been limited to stochastic flows with smooth probability distributions. This paper addresses these limitations by formulating a one-dimensional stochastic Galerkin shallow flow model using a low-order Wiener-Hermite Polynomial Chaos expansion with a finite volume Godunov-type approach, incorporating the surface gradient method to guarantee well-balancing. Preservation of a lake-at-rest over uncertain topography is verified analytically and numerically. The model is also assessed using flows with discontinuous and highly non-Gaussian probability distributions. Prescribing constant inflow over uncertain topography, the model converges on a steady-state flow that is subcritical or transcritical depending on the topography elevation. Using only four Wiener-Hermite basis functions, the model produces probability distributions comparable to those from a Monte Carlo reference simulation with 2000 iterations, while executing about 100 times faster. Accompanying model software and simulation data is openly available online.

==> eta.tex <==
\subsection{$\eta$-form (might not include)}
The flow can be expressed in terms of water height $h$, or water elevation $\eta = h + z$ where $z$ is the bed elevation, resulting in two formulations called $h$-form and $\eta$-form.

For the $\eta$-form model the flow, flux and source term are \citep{liang-borthwick2009}
\begin{subequations}
\begin{align}
    \flow &= \left[ \eta, q \right]^\T \\
    \flux &= \left[ q, \frac{q^2}{\eta - z} +
            \frac{g}{2}\left(\eta^2 - 2\eta z \right) \right]^\T \\
    \source &= \left[ 0, -g \eta \frac{\dee z}{\dee x} \right]^\T
\end{align}
\end{subequations}

For the $\eta$-form model, the source term $\source_i$ is \citep{liang-borthwick2009}
\begin{align}
    \source_i = \left[ 0, -g \eta_i \frac{\Delta z_i}{\Delta x} \right]^\T \label{eqn:source-eta}
\end{align}
where $\Delta z_i$ is calculated based on the averaged bed elevation at interfaces.  The averaged bed elevation $z_{i+1/2}^\pm$ at interface $i+1/2$ is
\begin{align}
z_{i+1/2}^\pm = \frac{z_i + z_{i+1}}{2} \label{eqn:z-interface}
\end{align}
and the change in bed elevation $\Delta z_i$ over element $i$ is
\begin{align}
    \Delta z_i = z_{i+1/2}^\pm - z_{i-1/2}^\pm \label{eqn:delta-z}
\end{align}

The stochastic source term for the $\eta$-form model is derived from equation~\eqref{eqn:source-eta},
\begin{align}
    \Ensemble{\source_i \pcbasis_l} = \left[ 0,
    -\frac{g}{\Delta x} \sum_{p=0}^P \sum_{q=0}^P \eta_{i,p}
    \Delta z_{i,q}
    \Ensemble{\pcbasis_p \pcbasis_q \pcbasis_l}
    \right]^\T \label{eqn:pc-source-eta}
\end{align}
where $\Delta z_{i,q} = z_{i+1/2,q}^\pm - z_{i-1/2,q}^\pm$ and $z_{i+1/2,q}^\pm = (z_{i,q}+z_{i+1,q})/2$.
The double summation in equation~\eqref{eqn:pc-source-eta} is a result of the tensor product that arises from the polynomial chaos expansions of water elevation $\eta$ and bed elevation $z$.


